A census of face-transitive surfaces

A face-transitive surface is a triangulated 2-dimensional manifold whose automorphism group acts transitively on its set of triangles. In this paper, we investigate this class of highly symmetric surface triangulations. We identify seven types of such face-transitive surfaces, splitting up further into a total of thirteen sub-types, distinguished by how their automorphism groups act on them. We use these theoretical results to compute a census of face-transitive surfaces with up to 1280 faces by constructing suitable cycle double covers of cubic node-transitive graphs.

==> sections/dataftorientable.tex <==
\newpage
\subsection{Data: Face-transitive surfaces with respect to vertex-face types and Euler characteristics}

\label{f1}

This section contains some information about the census of face-transitive surfaces contained in \cite{facetransitivesurfaces}. We refer the reader to \cite[Section 6.3]{facetransitivesurfaces} for a description of how to read the below tables.
\subsubsection{Data of orientable face-transitive surfaces with at most \texorpdfstring{$1280$}{1280} faces}

 \begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{2}$ &$2$ & $642$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $3$ \\  
$\textbf{0}$ &$14$ & $45$ & $164$ & $0$ & $565$ & $54013$ & $0$ & $0$ & $0$ & $2393$ & $175$ & $0$ & $36$ \\  
$\textbf{-2}$ &$2$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-4}$ &$6$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-6}$ &$5$ & $6$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-8}$ &$8$ & $9$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $1$ \\  
$\textbf{-10}$ &$6$ & $5$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $1$ \\  
$\textbf{-12}$ &$6$ & $4$ & $2$ & $1$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-14}$ &$4$ & $4$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-16}$ &$15$ & $22$ & $0$ & $0$ & $7$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-18}$ &$18$ & $19$ & $4$ & $1$ & $8$ & $1$ & $1$ & $1$ & $0$ & $2$ & $1$ & $0$ & $2$ \\  
$\textbf{-20}$ &$5$ & $5$ & $3$ & $0$ & $4$ & $2$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-22}$ &$4$ & $1$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-24}$ &$21$ & $8$ & $0$ & $0$ & $18$ & $2$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $2$ \\  
$\textbf{-26}$ &$3$ & $6$ & $1$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $3$ \\  
$\textbf{-28}$ &$13$ & $9$ & $1$ & $0$ & $3$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $2$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-30}$ &$11$ & $8$ & $1$ & $2$ & $6$ & $2$ & $1$ & $1$ & $0$ & $3$ & $0$ & $0$ & $1$ \\  
$\textbf{-32}$ &$26$ & $29$ & $4$ & $1$ & $25$ & $6$ & $4$ & $0$ & $0$ & $3$ & $1$ & $0$ & $1$ \\  
$\textbf{-34}$ &$4$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-36}$ &$23$ & $19$ & $3$ & $3$ & $14$ & $4$ & $1$ & $1$ & $0$ & $1$ & $0$ & $1$ & $0$ \\  
$\textbf{-38}$ &$4$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-40}$ &$25$ & $21$ & $6$ & $3$ & $15$ & $1$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $1$ \\  
$\textbf{-42}$ &$7$ & $8$ & $6$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $2$ \\  
$\textbf{-44}$ &$6$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-46}$ &$9$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-48}$ &$46$ & $24$ & $3$ & $0$ & $67$ & $4$ & $0$ & $1$ & $0$ & $6$ & $0$ & $0$ & $2$ \\  
$\textbf{-50}$ &$5$ & $6$ & $1$ & $3$ & $3$ & $4$ & $3$ & $2$ & $0$ & $0$ & $0$ & $1$ & $2$ \\  
$\textbf{-52}$ &$7$ & $3$ & $6$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-54}$ &$28$ & $23$ & $4$ & $0$ & $25$ & $4$ & $1$ & $0$ & $0$ & $4$ & $2$ & $0$ & $3$ \\  
$\textbf{-56}$ &$32$ & $12$ & $2$ & $0$ & $13$ & $4$ & $0$ & $4$ & $1$ & $4$ & $0$ & $0$ & $0$ \\  
$\textbf{-58}$ &$6$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-60}$ &$14$ & $11$ & $3$ & $0$ & $20$ & $12$ & $6$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-62}$ &$3$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-64}$ &$65$ & $60$ & $8$ & $2$ & $83$ & $14$ & $29$ & $1$ & $0$ & $15$ & $1$ & $0$ & $3$ \\  
$\textbf{-66}$ &$5$ & $3$ & $4$ & $0$ & $4$ & $1$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-68}$ &$5$ & $2$ & $5$ & $1$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-70}$ &$16$ & $15$ & $0$ & $1$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-72}$ &$51$ & $34$ & $2$ & $2$ & $82$ & $18$ & $10$ & $3$ & $1$ & $11$ & $1$ & $0$ & $2$ \\  
$\textbf{-74}$ &$3$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-76}$ &$7$ & $3$ & $1$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-78}$ &$15$ & $7$ & $6$ & $1$ & $3$ & $1$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ \\  
$\textbf{-80}$ &$58$ & $44$ & $21$ & $7$ & $50$ & $7$ & $2$ & $1$ & $0$ & $5$ & $0$ & $1$ & $2$ \\  
$\textbf{-82}$ &$5$ & $1$ & $6$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-84}$ &$15$ & $12$ & $6$ & $0$ & $15$ & $7$ & $0$ & $2$ & $2$ & $4$ & $1$ & $0$ & $1$ \\  
$\textbf{-86}$ &$4$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-88}$ &$37$ & $12$ & $2$ & $1$ & $11$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $3$ \\  
$\textbf{-90}$ &$36$ & $24$ & $7$ & $2$ & $21$ & $3$ & $0$ & $0$ & $0$ & $5$ & $1$ & $0$ & $2$ \\  
$\textbf{-92}$ &$7$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-94}$ &$6$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-96}$ &$107$ & $62$ & $8$ & $5$ & $204$ & $33$ & $32$ & $5$ & $3$ & $26$ & $0$ & $0$ & $3$ \\  
$\textbf{-98}$ &$6$ & $5$ & $7$ & $1$ & $6$ & $5$ & $5$ & $1$ & $0$ & $2$ & $0$ & $0$ & $1$ \\  
$\textbf{-100}$ &$17$ & $13$ & $15$ & $2$ & $11$ & $3$ & $4$ & $2$ & $0$ & $0$ & $1$ & $0$ & $0$ \\  
$\textbf{-102}$ &$7$ & $1$ & $5$ & $0$ & $5$ & $2$ & $0$ & $4$ & $0$ & $1$ & $0$ & $0$ & $2$ \\  
$\textbf{-104}$ &$27$ & $6$ & $8$ & $0$ & $7$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-106}$ &$5$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-108}$ &$45$ & $33$ & $7$ & $3$ & $50$ & $25$ & $10$ & $3$ & $1$ & $11$ & $0$ & $1$ & $1$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-110}$ &$12$ & $3$ & $6$ & $2$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-112}$ &$78$ & $28$ & $2$ & $6$ & $41$ & $11$ & $0$ & $8$ & $3$ & $6$ & $0$ & $0$ & $0$ \\  
$\textbf{-114}$ &$7$ & $2$ & $10$ & $0$ & $3$ & $2$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ \\  
$\textbf{-116}$ &$9$ & $1$ & $9$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-118}$ &$7$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-120}$ &$38$ & $18$ & $10$ & $0$ & $109$ & $32$ & $20$ & $0$ & $2$ & $21$ & $0$ & $0$ & $0$ \\  
$\textbf{-122}$ &$4$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-124}$ &$14$ & $8$ & $0$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-126}$ &$43$ & $19$ & $15$ & $4$ & $24$ & $7$ & $0$ & $0$ & $0$ & $3$ & $1$ & $0$ & $0$ \\  
$\textbf{-128}$ &$145$ & $87$ & $19$ & $13$ & $271$ & $76$ & $175$ & $6$ & $3$ & $44$ & $0$ & $0$ & $3$ \\  
$\textbf{-130}$ &$9$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-132}$ &$19$ & $5$ & $0$ & $0$ & $17$ & $5$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-134}$ &$5$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-136}$ &$31$ & $12$ & $6$ & $1$ & $12$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $3$ \\  
$\textbf{-138}$ &$8$ & $4$ & $1$ & $0$ & $4$ & $3$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-140}$ &$5$ & $11$ & $4$ & $0$ & $17$ & $0$ & $0$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-142}$ &$8$ & $1$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-144}$ &$166$ & $73$ & $10$ & $9$ & $285$ & $61$ & $69$ & $15$ & $8$ & $43$ & $1$ & $1$ & $5$ \\  
$\textbf{-146}$ &$4$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-148}$ &$16$ & $5$ & $5$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-150}$ &$31$ & $15$ & $0$ & $3$ & $28$ & $9$ & $0$ & $1$ & $0$ & $5$ & $0$ & $0$ & $2$ \\  
$\textbf{-152}$ &$30$ & $9$ & $2$ & $1$ & $10$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-154}$ &$14$ & $6$ & $4$ & $4$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-156}$ &$25$ & $3$ & $9$ & $0$ & $16$ & $6$ & $0$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-158}$ &$4$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-160}$ &$148$ & $93$ & $36$ & $13$ & $187$ & $30$ & $19$ & $0$ & $1$ & $13$ & $0$ & $1$ & $2$ \\  
$\textbf{-162}$ &$43$ & $44$ & $13$ & $2$ & $57$ & $36$ & $10$ & $1$ & $1$ & $20$ & $0$ & $0$ & $5$ \\  
$\textbf{-164}$ &$6$ & $2$ & $3$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-166}$ &$5$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-168}$ &$56$ & $31$ & $7$ & $1$ & $61$ & $24$ & $7$ & $10$ & $2$ & $18$ & $1$ & $0$ & $1$ \\  
$\textbf{-170}$ &$5$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-172}$ &$4$ & $2$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-174}$ &$9$ & $1$ & $1$ & $1$ & $1$ & $4$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-176}$ &$135$ & $21$ & $2$ & $2$ & $23$ & $4$ & $0$ & $8$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-178}$ &$5$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-180}$ &$47$ & $20$ & $11$ & $3$ & $67$ & $51$ & $12$ & $3$ & $2$ & $22$ & $0$ & $0$ & $1$ \\  
$\textbf{-182}$ &$3$ & $1$ & $10$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $2$ \\  
$\textbf{-184}$ &$33$ & $8$ & $11$ & $1$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-186}$ &$11$ & $3$ & $6$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ \\  
$\textbf{-188}$ &$4$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-190}$ &$18$ & $4$ & $2$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $3$ \\  
$\textbf{-192}$ &$188$ & $93$ & $14$ & $9$ & $483$ & $148$ & $217$ & $13$ & $7$ & $94$ & $1$ & $0$ & $3$ \\  
$\textbf{-194}$ &$2$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-196}$ &$8$ & $11$ & $1$ & $2$ & $10$ & $7$ & $7$ & $4$ & $2$ & $2$ & $0$ & $0$ & $1$ \\  
$\textbf{-198}$ &$31$ & $30$ & $4$ & $0$ & $20$ & $7$ & $0$ & $0$ & $0$ & $9$ & $0$ & $0$ & $0$ \\  
$\textbf{-200}$ &$21$ & $19$ & $24$ & $2$ & $57$ & $23$ & $16$ & $6$ & $1$ & $8$ & $0$ & $0$ & $0$ \\  
$\textbf{-202}$ &$3$ & $1$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-204}$ &$18$ & $5$ & $7$ & $1$ & $8$ & $8$ & $0$ & $8$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-206}$ &$3$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-208}$ &$120$ & $35$ & $13$ & $8$ & $17$ & $5$ & $0$ & $10$ & $0$ & $0$ & $0$ & $0$ & $4$ \\  
$\textbf{-210}$ &$1$ & $2$ & $9$ & $0$ & $3$ & $6$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ \\  
$\textbf{-212}$ &$4$ & $3$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-214}$ &$6$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-216}$ &$100$ & $40$ & $3$ & $3$ & $134$ & $92$ & $57$ & $8$ & $3$ & $59$ & $1$ & $0$ & $4$ \\  
$\textbf{-218}$ &$3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-220}$ &$6$ & $3$ & $3$ & $0$ & $4$ & $1$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-222}$ &$8$ & $3$ & $7$ & $1$ & $0$ & $5$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ \\  
$\textbf{-224}$ &$182$ & $67$ & $15$ & $17$ & $102$ & $49$ & $17$ & $16$ & $7$ & $9$ & $1$ & $0$ & $0$ \\  
$\textbf{-226}$ &$3$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-228}$ &$9$ & $5$ & $5$ & $0$ & $12$ & $9$ & $0$ & $2$ & $0$ & $1$ & $0$ & $0$ & $2$ \\  
$\textbf{-230}$ &$6$ & $2$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-232}$ &$33$ & $10$ & $1$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-234}$ &$11$ & $20$ & $8$ & $3$ & $6$ & $7$ & $0$ & $0$ & $2$ & $3$ & $1$ & $0$ & $0$ \\  
$\textbf{-236}$ &$2$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-238}$ &$11$ & $7$ & $0$ & $2$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-240}$ &$105$ & $24$ & $20$ & $2$ & $301$ & $98$ & $65$ & $4$ & $3$ & $49$ & $0$ & $0$ & $2$ \\  
$\textbf{-242}$ &$0$ & $4$ & $13$ & $0$ & $4$ & $5$ & $9$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-244}$ &$6$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-246}$ &$2$ & $2$ & $4$ & $0$ & $1$ & $6$ & $0$ & $4$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-248}$ &$23$ & $6$ & $1$ & $0$ & $1$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-250}$ &$13$ & $12$ & $3$ & $3$ & $0$ & $2$ & $3$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-252}$ &$25$ & $20$ & $18$ & $6$ & $27$ & $48$ & $16$ & $14$ & $5$ & $5$ & $1$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-254}$ &$2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-256}$ &$341$ & $126$ & $12$ & $35$ & $704$ & $302$ & $781$ & $18$ & $11$ & $143$ & $2$ & $1$ & $7$ \\  
$\textbf{-258}$ &$4$ & $1$ & $1$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ \\  
$\textbf{-260}$ &$6$ & $5$ & $13$ & $2$ & $5$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-262}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-264}$ &$55$ & $13$ & $4$ & $1$ & $52$ & $11$ & $0$ & $4$ & $0$ & $5$ & $0$ & $0$ & $1$ \\  
$\textbf{-266}$ &$1$ & $1$ & $7$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-268}$ &$7$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-270}$ &$40$ & $38$ & $10$ & $8$ & $26$ & $26$ & $3$ & $0$ & $0$ & $16$ & $1$ & $0$ & $1$ \\  
$\textbf{-272}$ &$61$ & $20$ & $12$ & $2$ & $14$ & $7$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-274}$ &$0$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-276}$ &$5$ & $5$ & $0$ & $0$ & $2$ & $11$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-278}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-280}$ &$13$ & $13$ & $14$ & $0$ & $43$ & $7$ & $0$ & $10$ & $2$ & $4$ & $0$ & $1$ & $0$ \\  
$\textbf{-282}$ &$7$ & $0$ & $1$ & $0$ & $1$ & $7$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-284}$ &$6$ & $1$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-286}$ &$0$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-288}$ &$365$ & $97$ & $16$ & $13$ & $337$ & $278$ & $355$ & $37$ & $36$ & $130$ & $0$ & $0$ & $7$ \\  
$\textbf{-290}$ &$5$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-292}$ &$11$ & $4$ & $4$ & $1$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-294}$ &$1$ & $8$ & $13$ & $1$ & $6$ & $14$ & $6$ & $2$ & $0$ & $1$ & $1$ & $0$ & $1$ \\  
$\textbf{-296}$ &$21$ & $14$ & $3$ & $0$ & $5$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-298}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-300}$ &$13$ & $4$ & $6$ & $0$ & $16$ & $57$ & $13$ & $8$ & $0$ & $9$ & $1$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-304}$ &$54$ & $20$ & $1$ & $0$ & $13$ & $8$ & $0$ & $8$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-306}$ &$2$ & $16$ & $5$ & $0$ & $7$ & $10$ & $0$ & $4$ & $0$ & $3$ & $0$ & $0$ & $0$ \\  
$\textbf{-308}$ &$1$ & $5$ & $1$ & $2$ & $0$ & $0$ & $0$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-310}$ &$10$ & $4$ & $2$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-312}$ &$105$ & $8$ & $10$ & $0$ & $12$ & $13$ & $0$ & $12$ & $0$ & $5$ & $1$ & $0$ & $0$ \\  
$\textbf{-314}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-316}$ &$3$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-318}$ &$3$ & $1$ & $1$ & $1$ & $1$ & $8$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-320}$ &$267$ & $91$ & $40$ & $47$ & $474$ & $143$ & $125$ & $6$ & $3$ & $71$ & $0$ & $1$ & $2$ \\  
$\textbf{-322}$ &$1$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-324}$ &$21$ & $16$ & $6$ & $0$ & $33$ & $116$ & $25$ & $14$ & $7$ & $37$ & $0$ & $0$ & $2$ \\  
$\textbf{-328}$ &$25$ & $6$ & $4$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-330}$ &$3$ & $4$ & $10$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-332}$ &$5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-336}$ &$121$ & $39$ & $12$ & $1$ & $93$ & $23$ & $0$ & $22$ & $2$ & $7$ & $1$ & $1$ & $2$ \\  
$\textbf{-338}$ &$1$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-340}$ &$7$ & $7$ & $0$ & $1$ & $14$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-342}$ &$12$ & $9$ & $9$ & $1$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-344}$ &$19$ & $6$ & $0$ & $0$ & $4$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-348}$ &$2$ & $1$ & $7$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-350}$ &$8$ & $13$ & $2$ & $8$ & $17$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-352}$ &$218$ & $26$ & $3$ & $19$ & $41$ & $14$ & $0$ & $16$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-354}$ &$0$ & $0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-356}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-360}$ &$133$ & $19$ & $14$ & $10$ & $103$ & $81$ & $11$ & $11$ & $1$ & $29$ & $0$ & $0$ & $0$ \\  
$\textbf{-364}$ &$4$ & $2$ & $0$ & $1$ & $0$ & $5$ & $0$ & $8$ & $0$ & $6$ & $0$ & $0$ & $0$ \\  
$\textbf{-366}$ &$5$ & $2$ & $2$ & $1$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-368}$ &$37$ & $11$ & $2$ & $3$ & $2$ & $10$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-370}$ &$7$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-372}$ &$5$ & $0$ & $9$ & $0$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-374}$ &$0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-376}$ &$2$ & $1$ & $1$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-378}$ &$0$ & $10$ & $10$ & $5$ & $0$ & $16$ & $0$ & $0$ & $0$ & $12$ & $3$ & $0$ & $1$ \\  
$\textbf{-380}$ &$8$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-384}$ &$144$ & $39$ & $0$ & $8$ & $208$ & $173$ & $265$ & $16$ & $9$ & $41$ & $0$ & $0$ & $0$ \\  
$\textbf{-388}$ &$0$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-390}$ &$4$ & $1$ & $5$ & $0$ & $5$ & $12$ & $0$ & $0$ & $0$ & $10$ & $0$ & $0$ & $1$ \\  
$\textbf{-392}$ &$5$ & $2$ & $2$ & $0$ & $1$ & $22$ & $3$ & $21$ & $1$ & $4$ & $0$ & $0$ & $0$ \\  
$\textbf{-394}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-396}$ &$12$ & $1$ & $2$ & $0$ & $1$ & $6$ & $0$ & $1$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-400}$ &$5$ & $12$ & $20$ & $4$ & $37$ & $56$ & $35$ & $6$ & $4$ & $14$ & $0$ & $0$ & $0$ \\  
$\textbf{-402}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-404}$ &$1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-406}$ &$6$ & $4$ & $0$ & $5$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-408}$ &$52$ & $7$ & $6$ & $3$ & $21$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-410}$ &$11$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-414}$ &$0$ & $1$ & $8$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-416}$ &$15$ & $12$ & $8$ & $5$ & $13$ & $17$ & $0$ & $21$ & $0$ & $2$ & $0$ & $1$ & $2$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-418}$ &$1$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-420}$ &$3$ & $1$ & $2$ & $0$ & $6$ & $0$ & $0$ & $7$ & $0$ & $1$ & $1$ & $0$ & $0$ \\  
$\textbf{-424}$ &$5$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-426}$ &$0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-428}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-430}$ &$6$ & $4$ & $3$ & $5$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-432}$ &$24$ & $17$ & $6$ & $2$ & $30$ & $26$ & $11$ & $2$ & $12$ & $25$ & $0$ & $0$ & $2$ \\  
$\textbf{-434}$ &$0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-436}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-440}$ &$1$ & $2$ & $4$ & $0$ & $15$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-442}$ &$0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-444}$ &$2$ & $1$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-448}$ &$19$ & $15$ & $0$ & $1$ & $44$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-450}$ &$0$ & $5$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-456}$ &$16$ & $4$ & $0$ & $1$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-460}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-462}$ &$0$ & $0$ & $2$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-464}$ &$6$ & $4$ & $4$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-468}$ &$0$ & $1$ & $5$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ \\  
$\textbf{-470}$ &$1$ & $1$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-472}$ &$0$ & $0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-480}$ &$6$ & $6$ & $3$ & $0$ & $17$ & $11$ & $3$ & $3$ & $7$ & $12$ & $0$ & $0$ & $0$ \\  
$\textbf{-488}$ &$4$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-490}$ &$1$ & $3$ & $4$ & $3$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-496}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $8$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-500}$ &$0$ & $2$ & $2$ & $0$ & $1$ & $10$ & $0$ & $2$ & $0$ & $5$ & $0$ & $0$ & $0$ \\  
$\textbf{-504}$ &$0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $1$ & $6$ & $3$ & $0$ & $0$ & $2$ \\  
$\textbf{-510}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-512}$ &$0$ & $0$ & $1$ & $0$ & $0$ & $4$ & $8$ & $0$ & $2$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-520}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-528}$ &$0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-550}$ &$0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
\end{ttabular} 
\caption{Numbers of computed orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\subsubsection{Data of non-orientable face-transitive surfaces with at most \texorpdfstring{$1280$}{1280} faces}

  \begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{1}$ &$2$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-2}$ &$2$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-3}$ &$2$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-4}$ &$3$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-5}$ &$2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-6}$ &$1$ & $2$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-7}$ &$2$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-8}$ &$6$ & $7$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-9}$ &$1$ & $3$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-10}$ &$2$ & $4$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-11}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-12}$ &$3$ & $3$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-13}$ &$1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-14}$ &$4$ & $5$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-15}$ &$4$ & $3$ & $0$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $1$ \\  
$\textbf{-16}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-17}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-18}$ &$3$ & $3$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-20}$ &$4$ & $4$ & $0$ & $2$ & $6$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-21}$ &$3$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-23}$ &$2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-24}$ &$4$ & $4$ & $0$ & $0$ & $11$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-25}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-26}$ &$2$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-27}$ &$5$ & $5$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-28}$ &$12$ & $9$ & $0$ & $0$ & $7$ & $0$ & $0$ & $0$ & $1$ & $4$ & $0$ & $0$ & $0$ \\  
$\textbf{-29}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-30}$ &$2$ & $2$ & $0$ & $0$ & $6$ & $0$ & $5$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ \\  
$\textbf{-32}$ &$7$ & $4$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-33}$ &$0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-34}$ &$1$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-35}$ &$5$ & $6$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-36}$ &$4$ & $4$ & $0$ & $0$ & $10$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-38}$ &$2$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-39}$ &$4$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-40}$ &$4$ & $4$ & $0$ & $0$ & $11$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-41}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-42}$ &$6$ & $9$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ \\  
$\textbf{-44}$ &$5$ & $8$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-45}$ &$6$ & $9$ & $0$ & $1$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-47}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-48}$ &$7$ & $13$ & $0$ & $3$ & $30$ & $0$ & $8$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ \\  
$\textbf{-49}$ &$1$ & $2$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-50}$ &$9$ & $4$ & $0$ & $0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-51}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-53}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-54}$ &$3$ & $10$ & $0$ & $0$ & $12$ & $0$ & $6$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-55}$ &$1$ & $7$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-56}$ &$11$ & $8$ & $0$ & $0$ & $9$ & $0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-58}$ &$4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-59}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-60}$ &$5$ & $9$ & $0$ & $0$ & $33$ & $0$ & $6$ & $0$ & $1$ & $7$ & $0$ & $0$ & $0$ \\  
$\textbf{-62}$ &$5$ & $7$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-63}$ &$6$ & $5$ & $0$ & $1$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-64}$ &$10$ & $6$ & $0$ & $0$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-65}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-66}$ &$1$ & $1$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-68}$ &$6$ & $5$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-70}$ &$11$ & $13$ & $0$ & $0$ & $11$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-71}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-72}$ &$2$ & $3$ & $0$ & $0$ & $22$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-74}$ &$2$ & $1$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-75}$ &$3$ & $4$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-76}$ &$6$ & $4$ & $0$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-77}$ &$3$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-78}$ &$1$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-80}$ &$21$ & $13$ & $0$ & $1$ & $22$ & $0$ & $1$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ \\  
$\textbf{-81}$ &$5$ & $5$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-82}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-83}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-84}$ &$8$ & $21$ & $0$ & $0$ & $22$ & $0$ & $6$ & $0$ & $1$ & $9$ & $0$ & $0$ & $2$ \\  
$\textbf{-86}$ &$3$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-88}$ &$12$ & $5$ & $0$ & $1$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-89}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-90}$ &$5$ & $8$ & $0$ & $1$ & $24$ & $0$ & $2$ & $0$ & $0$ & $8$ & $0$ & $0$ & $0$ \\  
$\textbf{-91}$ &$0$ & $6$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $2$ \\  
$\textbf{-92}$ &$4$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-95}$ &$7$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-96}$ &$11$ & $15$ & $0$ & $0$ & $54$ & $0$ & $24$ & $0$ & $2$ & $12$ & $0$ & $0$ & $0$ \\  
$\textbf{-98}$ &$3$ & $2$ & $0$ & $0$ & $10$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-99}$ &$13$ & $14$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ \\  
$\textbf{-100}$ &$3$ & $1$ & $0$ & $0$ & $10$ & $0$ & $3$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-101}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-102}$ &$6$ & $4$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-104}$ &$14$ & $16$ & $0$ & $4$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $3$ \\  
$\textbf{-105}$ &$0$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-106}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-107}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-108}$ &$4$ & $10$ & $0$ & $0$ & $38$ & $0$ & $10$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-110}$ &$2$ & $11$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ \\  
$\textbf{-111}$ &$0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-112}$ &$10$ & $6$ & $0$ & $2$ & $33$ & $0$ & $6$ & $0$ & $1$ & $4$ & $0$ & $0$ & $0$ \\  
$\textbf{-113}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-114}$ &$8$ & $2$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-116}$ &$9$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-117}$ &$4$ & $11$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-118}$ &$0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-119}$ &$4$ & $4$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-120}$ &$12$ & $7$ & $0$ & $0$ & $73$ & $0$ & $10$ & $0$ & $2$ & $11$ & $0$ & $0$ & $0$ \\  
$\textbf{-121}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-122}$ &$2$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-123}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-124}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-125}$ &$1$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-126}$ &$6$ & $2$ & $0$ & $2$ & $26$ & $0$ & $13$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-128}$ &$10$ & $14$ & $0$ & $0$ & $21$ & $0$ & $16$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-130}$ &$2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-131}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-132}$ &$5$ & $11$ & $0$ & $2$ & $9$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-134}$ &$2$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-135}$ &$8$ & $13$ & $0$ & $2$ & $10$ & $0$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-136}$ &$4$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-137}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-138}$ &$5$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-139}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-140}$ &$11$ & $18$ & $0$ & $0$ & $26$ & $0$ & $0$ & $0$ & $1$ & $2$ & $0$ & $1$ & $0$ \\  
$\textbf{-142}$ &$2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-143}$ &$3$ & $8$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-144}$ &$20$ & $13$ & $0$ & $0$ & $55$ & $0$ & $11$ & $0$ & $0$ & $6$ & $0$ & $0$ & $1$ \\  
$\textbf{-145}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-146}$ &$3$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-147}$ &$2$ & $2$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-148}$ &$9$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-149}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-150}$ &$8$ & $6$ & $0$ & $1$ & $22$ & $0$ & $3$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ \\  
$\textbf{-152}$ &$12$ & $9$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-153}$ &$9$ & $10$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-154}$ &$5$ & $7$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-155}$ &$3$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-156}$ &$8$ & $2$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-158}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-159}$ &$3$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-160}$ &$20$ & $21$ & $0$ & $3$ & $38$ & $0$ & $8$ & $1$ & $0$ & $8$ & $0$ & $0$ & $0$ \\  
$\textbf{-162}$ &$3$ & $10$ & $0$ & $1$ & $25$ & $0$ & $15$ & $1$ & $1$ & $13$ & $0$ & $0$ & $0$ \\  
$\textbf{-164}$ &$6$ & $3$ & $0$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-165}$ &$2$ & $6$ & $0$ & $0$ & $5$ & $0$ & $2$ & $0$ & $0$ & $7$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-168}$ &$11$ & $21$ & $0$ & $0$ & $60$ & $0$ & $14$ & $0$ & $2$ & $5$ & $0$ & $1$ & $2$ \\  
$\textbf{-169}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-170}$ &$3$ & $6$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-171}$ &$6$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-172}$ &$4$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-174}$ &$3$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-175}$ &$5$ & $7$ & $0$ & $1$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-176}$ &$24$ & $7$ & $0$ & $2$ & $12$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-178}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-180}$ &$8$ & $11$ & $0$ & $1$ & $75$ & $0$ & $12$ & $0$ & $1$ & $14$ & $0$ & $0$ & $0$ \\  
$\textbf{-182}$ &$7$ & $7$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $10$ & $0$ & $0$ & $0$ \\  
$\textbf{-183}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-184}$ &$4$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-186}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-188}$ &$0$ & $1$ & $0$ & $2$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-189}$ &$7$ & $16$ & $0$ & $4$ & $9$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-190}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-192}$ &$5$ & $6$ & $0$ & $1$ & $84$ & $0$ & $44$ & $0$ & $4$ & $29$ & $0$ & $0$ & $0$ \\  
$\textbf{-194}$ &$1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-195}$ &$3$ & $8$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ \\  
$\textbf{-196}$ &$6$ & $3$ & $0$ & $0$ & $19$ & $0$ & $3$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-198}$ &$5$ & $20$ & $0$ & $0$ & $26$ & $0$ & $1$ & $0$ & $0$ & $12$ & $0$ & $0$ & $0$ \\  
$\textbf{-200}$ &$5$ & $9$ & $0$ & $0$ & $32$ & $0$ & $1$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ \\  
$\textbf{-202}$ &$0$ & $0$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-203}$ &$3$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-204}$ &$9$ & $6$ & $0$ & $0$ & $13$ & $0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $1$ \\  
$\textbf{-206}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-207}$ &$13$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-208}$ &$27$ & $19$ & $0$ & $1$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-209}$ &$0$ & $9$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-210}$ &$4$ & $12$ & $0$ & $0$ & $45$ & $0$ & $1$ & $0$ & $0$ & $3$ & $0$ & $0$ & $1$ \\  
$\textbf{-212}$ &$0$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-214}$ &$9$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-215}$ &$2$ & $3$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-216}$ &$6$ & $9$ & $0$ & $5$ & $63$ & $0$ & $23$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ \\  
$\textbf{-218}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-219}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-220}$ &$7$ & $5$ & $0$ & $0$ & $8$ & $0$ & $1$ & $0$ & $0$ & $12$ & $0$ & $0$ & $2$ \\  
$\textbf{-222}$ &$1$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-224}$ &$12$ & $37$ & $0$ & $7$ & $41$ & $0$ & $24$ & $0$ & $2$ & $13$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-225}$ &$1$ & $2$ & $0$ & $0$ & $9$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-226}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-227}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-228}$ &$4$ & $12$ & $0$ & $0$ & $16$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-230}$ &$0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-231}$ &$2$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-232}$ &$3$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-234}$ &$3$ & $8$ & $0$ & $0$ & $23$ & $0$ & $1$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-236}$ &$0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-238}$ &$0$ & $0$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-240}$ &$8$ & $9$ & $0$ & $0$ & $125$ & $0$ & $68$ & $0$ & $3$ & $25$ & $0$ & $0$ & $0$ \\  
$\textbf{-242}$ &$0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-243}$ &$4$ & $10$ & $0$ & $0$ & $7$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-244}$ &$6$ & $2$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-245}$ &$0$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-246}$ &$0$ & $0$ & $0$ & $0$ & $7$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-248}$ &$2$ & $3$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-250}$ &$1$ & $1$ & $0$ & $0$ & $2$ & $0$ & $13$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-252}$ &$11$ & $5$ & $0$ & $0$ & $28$ & $0$ & $54$ & $0$ & $1$ & $11$ & $0$ & $0$ & $0$ \\  
$\textbf{-253}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-254}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-255}$ &$2$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $4$ \\  
$\textbf{-256}$ &$8$ & $5$ & $0$ & $6$ & $38$ & $0$ & $67$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-258}$ &$0$ & $1$ & $0$ & $1$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-259}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-260}$ &$7$ & $2$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-261}$ &$0$ & $3$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-264}$ &$4$ & $4$ & $0$ & $0$ & $35$ & $0$ & $1$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ \\  
$\textbf{-266}$ &$0$ & $1$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-267}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-268}$ &$3$ & $2$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-270}$ &$0$ & $2$ & $0$ & $0$ & $18$ & $0$ & $30$ & $0$ & $0$ & $13$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-271}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-272}$ &$11$ & $11$ & $0$ & $5$ & $31$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $3$ \\  
$\textbf{-273}$ &$1$ & $8$ & $0$ & $0$ & $5$ & $0$ & $5$ & $0$ & $0$ & $9$ & $0$ & $0$ & $1$ \\  
$\textbf{-274}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-275}$ &$1$ & $6$ & $0$ & $1$ & $10$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-276}$ &$0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-278}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-279}$ &$0$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-280}$ &$0$ & $9$ & $0$ & $0$ & $28$ & $0$ & $0$ & $0$ & $1$ & $7$ & $0$ & $0$ & $0$ \\  
$\textbf{-282}$ &$2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-284}$ &$1$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-285}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-286}$ &$0$ & $9$ & $0$ & $1$ & $12$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-287}$ &$4$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-288}$ &$5$ & $8$ & $0$ & $1$ & $97$ & $0$ & $55$ & $4$ & $3$ & $41$ & $0$ & $0$ & $0$ \\  
$\textbf{-290}$ &$3$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-291}$ &$0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-292}$ &$13$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-294}$ &$0$ & $6$ & $0$ & $0$ & $22$ & $0$ & $2$ & $2$ & $1$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-296}$ &$2$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-297}$ &$15$ & $9$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-298}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-299}$ &$2$ & $13$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-300}$ &$0$ & $8$ & $0$ & $2$ & $21$ & $0$ & $23$ & $0$ & $1$ & $7$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-302}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-303}$ &$0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-304}$ &$2$ & $8$ & $0$ & $1$ & $7$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-306}$ &$0$ & $2$ & $0$ & $0$ & $6$ & $0$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-308}$ &$0$ & $4$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-310}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-312}$ &$5$ & $20$ & $0$ & $0$ & $13$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ \\  
$\textbf{-314}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-315}$ &$8$ & $6$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-316}$ &$2$ & $3$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-318}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-319}$ &$4$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-320}$ &$2$ & $1$ & $0$ & $0$ & $28$ & $0$ & $18$ & $1$ & $0$ & $17$ & $0$ & $0$ & $0$ \\  
$\textbf{-322}$ &$0$ & $5$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-323}$ &$0$ & $7$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-324}$ &$2$ & $7$ & $0$ & $1$ & $34$ & $0$ & $49$ & $0$ & $0$ & $7$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-325}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-328}$ &$8$ & $1$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-329}$ &$0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-330}$ &$5$ & $1$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-331}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-332}$ &$5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-333}$ &$4$ & $4$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-335}$ &$7$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-336}$ &$3$ & $4$ & $0$ & $0$ & $55$ & $0$ & $11$ & $0$ & $1$ & $11$ & $0$ & $0$ & $0$ \\  
$\textbf{-338}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-339}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-340}$ &$4$ & $6$ & $0$ & $0$ & $22$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-342}$ &$1$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-344}$ &$4$ & $4$ & $0$ & $2$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-348}$ &$6$ & $8$ & $0$ & $0$ & $10$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-350}$ &$0$ & $2$ & $0$ & $3$ & $14$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-351}$ &$11$ & $14$ & $0$ & $7$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-352}$ &$0$ & $0$ & $0$ & $0$ & $3$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-354}$ &$1$ & $5$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-357}$ &$0$ & $0$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-359}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-360}$ &$20$ & $3$ & $0$ & $0$ & $55$ & $0$ & $6$ & $0$ & $0$ & $9$ & $0$ & $0$ & $0$ \\  
$\textbf{-362}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-363}$ &$0$ & $1$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-364}$ &$0$ & $6$ & $0$ & $0$ & $2$ & $0$ & $5$ & $0$ & $0$ & $14$ & $0$ & $0$ & $0$ \\  
$\textbf{-366}$ &$1$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-368}$ &$1$ & $4$ & $0$ & $1$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-369}$ &$0$ & $4$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-370}$ &$5$ & $3$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-371}$ &$0$ & $5$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-372}$ &$0$ & $5$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-375}$ &$5$ & $2$ & $0$ & $1$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-376}$ &$0$ & $0$ & $0$ & $0$ & $7$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-377}$ &$0$ & $10$ & $0$ & $0$ & $9$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-378}$ &$0$ & $0$ & $0$ & $0$ & $9$ & $0$ & $7$ & $2$ & $0$ & $11$ & $0$ & $0$ & $0$ \\  
$\textbf{-380}$ &$7$ & $3$ & $0$ & $2$ & $2$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $3$ \\  
$\textbf{-384}$ &$2$ & $14$ & $0$ & $0$ & $86$ & $0$ & $107$ & $2$ & $1$ & $10$ & $0$ & $0$ & $0$ \\  
$\textbf{-385}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-386}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-387}$ &$1$ & $6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-388}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-390}$ &$0$ & $10$ & $0$ & $0$ & $14$ & $0$ & $0$ & $0$ & $0$ & $18$ & $0$ & $0$ & $0$ \\  
$\textbf{-392}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-394}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-395}$ &$1$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-396}$ &$0$ & $1$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-399}$ &$0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $4$ \\  
$\textbf{-400}$ &$2$ & $2$ & $0$ & $1$ & $37$ & $0$ & $8$ & $0$ & $1$ & $4$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-402}$ &$0$ & $2$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-403}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-404}$ &$0$ & $7$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-405}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $8$ & $0$ & $0$ & $0$ \\  
$\textbf{-408}$ &$2$ & $2$ & $0$ & $0$ & $19$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-410}$ &$6$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-411}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-413}$ &$0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-414}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-415}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-416}$ &$2$ & $0$ & $0$ & $0$ & $12$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-418}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-420}$ &$3$ & $7$ & $0$ & $1$ & $21$ & $0$ & $0$ & $0$ & $0$ & $3$ & $0$ & $0$ & $1$ \\  
$\textbf{-426}$ &$0$ & $0$ & $0$ & $0$ & $9$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-429}$ &$0$ & $4$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-430}$ &$0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-432}$ &$4$ & $2$ & $0$ & $1$ & $24$ & $0$ & $7$ & $0$ & $0$ & $5$ & $0$ & $0$ & $0$ \\  
$\textbf{-435}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-436}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-438}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-440}$ &$2$ & $3$ & $0$ & $1$ & $8$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-441}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-444}$ &$0$ & $2$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-447}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-448}$ &$4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ \\  
$\textbf{-450}$ &$0$ & $0$ & $0$ & $0$ & $11$ & $0$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-452}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-455}$ &$1$ & $2$ & $0$ & $2$ & $0$ & $0$ & $6$ & $0$ & $0$ & $3$ & $0$ & $0$ & $0$ \\  
$\textbf{-456}$ &$0$ & $0$ & $0$ & $0$ & $10$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-459}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $2$ & $0$ & $0$ & $0$ \\  
$\textbf{-460}$ &$0$ & $4$ & $0$ & $0$ & $10$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-468}$ &$0$ & $1$ & $0$ & $0$ & $1$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-470}$ &$0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-475}$ &$0$ & $5$ & $0$ & $0$ & $10$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $1$ \\  
$\textbf{-476}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $6$ & $0$ & $0$ & $0$ \\  
$\textbf{-480}$ &$0$ & $0$ & $0$ & $0$ & $1$ & $0$ & $39$ & $0$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-484}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-487}$ &$1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-492}$ &$0$ & $1$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
$\textbf{-496}$ &$0$ & $0$ & $0$ & $4$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular} 
\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types}
 \end{table}
\begin{table}[H]
 \centering 
 \begin{ttabular} 
 \textbf{$\chi(X)$} & $\textbf{(3,1)}$ & $\textbf{(2,2)}$ & $\textbf{(2,1).1}$ & $\textbf{(2,1).2}$ & $\textbf{(2,1).3}$  & $\textbf{(1,1).1}$ &
 $\textbf{(1,1).2}$ & $\textbf{(1,1).3}$ & $\textbf{(1,1).4}$ & $\textbf{(1,2)}$ & $\textbf{(1,3).1}$ & $\textbf{(1,3).2}$ & $\textbf{(1,6)}$ \\  
$\textbf{-500}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $10$ & $2$ & $0$ & $1$ & $0$ & $0$ & $0$ \\  
$\textbf{-512}$ &$0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $8$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ \\  
\end{ttabular}\caption{Numbers of computed non-orientable face-transitive surfaces with at most $1280$ faces with respect to their Euler characteristics and vertex-face types.\
}
 \end{table}
